LibEvolutionEval: A Benchmark and Study for Version-Specific Code Generation

Recent advancements in code completion models have primarily focused on local file contexts. However, these studies do not fully capture the complexity of real-world software development, which often requires the use of rapidly-evolving public libraries. To fill the gap, we introduce LibEvolutionEval, a detailed study requiring an understanding of library evolution to perform in-line code completion accurately. LibEvolutionEval provides a version-specific code-completion task comprised of eight libraries (torch, torchvision, scipy, pil, tqdm, pyyaml, matplotlib, and pandas) as they evolve over the year along with a detailed analysis of the evolution of two popular and well-maintained public libraries: PyTorch and Matplotlib. We evaluate popular public models and find that public library evolution significantly influences model performance. We explored mitigation methods by studying how retrieved version-specific library documentation and prompting can improve the model's capability in handling these fast-evolving packages, paving a promising future path in better handling fast-evolving libraries.

==> sections/1_introduction_old.tex <==
\section{Introduction}

Large Language Models for code (code LLMs) such as StarCoder~\citep{li2023starcoder}, StarCoder2~\citep{lozhkov2024starcoder}, CodeLlama~\citep{roziere2023code}, and Codex~\citep{chen2021evaluating} have significantly advanced developer productivity through enhanced code and function completion tasks. These models are not only pivotal in code completion but also in debugging, code summarization, and language translation for software development \citep{yan2023codetransocean, lachaux2020unsupervised, roziere2021leveraging, min2023beyond}.
Various studies have been done to evaluate these models with a focus on local files for context to enhance function completion~\citep{chen2021evaluating, ding2023static, athiwaratkun2022multi, ding2023crosscodeeval, jimenez2024swebench}. 
However, these studies do not fully encompass the complexities of real-world software development, which requires the use of public libraries. While some works perform code completion involving public libraries~\citep{liao2023context, zan2022cert}, use documentation of the library for prediction~\citep{qin2023toolllm}, and show that {zero shot}
code completions suffer from hallucinations~\citep{patil2023gorilla}, these works do not focus on the rapidly evolving nature of public libraries.

LLMs are likely to have encountered public libraries during their pretraining since they are trained on vast corpora of open-source code. However, these libraries evolve rapidly with the introduction, deprecation, and modification of APIs~\citep{mcdonnell2013empirical}.
These changes are not explicitly incorporated into these models. Thus, while LLM generations may be reasonable, they can be incorrect for the version under consideration, leading to version-dependent performance (refer to Figure~\ref{fig:context_example}). This dependence is significant as developers use different versions of the same library, for example, using the latest versions for new projects while using outdated versions for legacy code maintenance. Thus, the developer's experience using LLMs for code completion with public libraries can vary significantly based on their specific use case. Existing benchmarks and studies do not fully capture the performance of LLMs concerning public libraries, revealing a gap in our current evaluation of code LLMs.\looseness=-1

\begin{figure*}
    \centering
    \includegraphics[width=0.95\textwidth]{figures/figure1.png}
    \caption{This figure demonstrates a code completion scenario under \schemelong. The incomplete code snippet on the left requires the correct API method to solve a linear system specified by two PyTorch tensors. The Code LLM performs incorrect code completions due to version mismatch. 
    The version-specific documentation is a potential {augmentations} that can assist the LLM to perform correct and version-dependent completion.
    }
    \label{fig:context_example}
\end{figure*}


To address these challenges, we introduce \schemelong{}, a benchmark specifically designed to evaluate the performance of Code LLMs with respect to multiple versions of public libraries capturing their evolution over the years. \schemelong{} investigates "\emph{Does the performance of Code LLMs change as the library evolves?}” by providing a code-completion task focusing on 8 libraries (\emph{torch, torchvision, scipy, PIL, tqdm, pyyaml, matplotlib and pandas}) spanning five years with unique APIs for every year. 

Furthermore, we perform a detailed analysis using two popular libraries: \emph{PyTorch} and \emph{Matplotlib}. Both libraries were built sufficiently long ago, are widely used, and are still being actively developed. Constructing the evaluation examples can be done using different methods: Snippets from permissively licensed repositories from GitHub can be extracted, representing a \emph{realistic scenario} scenario of library use; 
Construction of examples can be done via a template and API documentation, offering a more \emph{controlled} way for evaluation and comparison.\looseness=-1

With the evolution of libraries, new relationships between APIs are introduced, while existing ones are altered. This raises an important question: \emph{Can Code LLMs effectively adapt to these evolving relationships?} One aspect of this challenge lies in comparing different types of completions—those guided by import statements and clear library prefixes, versus object-oriented references that do not explicitly include library-defined prefixes. Another key question emerging from evolution is "\textit{Does the addition, modification, or deprecation of APIs as libraries evolve make it more challenging for Code LLMs to perform accurate code completions?}" This requires tracking the life of the API as the documentation of the library evolves.  Thus, \schemelong{} offers meta-data to enhance version-specific code completions by providing version-specific API documentation which ensures that models can access the correct usage of APIs relevant to each library version to encourage the correct APIs for code completion. This enables \schemelong{} to assess the ability of code embedding models to retrieve accurate documentation as public libraries evolve rapidly. 

We conducted a comprehensive evaluation of widely used public Code LLMs.%~\citep{lozhkov2024starcoder, jiang2023mistral}. 
Our empirical findings underscore that the performance of Code LLMs in performing code completions exhibits substantial variation across different library versions. Notably, our use of \schemelong revealed insightful performance trends: these models tended to underperform in code completions that require APIs that were added/deleted/modified and excel in code completions that involve object-oriented references. Similarly, the efficacy of code embedding models in retrieving accurate documentation also demonstrates significant variability.
By highlighting these capabilities and limitations, \schemelong can serve as a positive influence for driving forward the development of code completion technologies for more sophisticated models that better handle evolving APIs.

